Application of Adversarial Examples to Physical ECG Signals

This work aims to assess the reality and feasibility of the adversarial attack against cardiac diagnosis system powered by machine learning algorithms. To this end, we introduce adversarial beats, which are adversarial perturbations tailored specifically against electrocardiograms (ECGs) beat-by-beat classification system. We first formulate an algorithm to generate adversarial examples for the ECG classification neural network model, and study its attack success rate. Next, to evaluate its feasibility in a physical environment, we mount a hardware attack by designing a malicious signal generator which injects adversarial beats into ECG sensor readings. To the best of our knowledge, our work is the first in evaluating the proficiency of adversarial examples for ECGs in a physical setup. Our real-world experiments demonstrate that adversarial beats successfully manipulated the diagnosis results 3-5 times out of 40 attempts throughout the course of 2 minutes. Finally, we discuss the overall feasibility and impact of the attack, by clearly defining motives and constraints of expected attackers along with our experimental results.

==> sections/XX_related.tex <==
\section{Related work}
\label{sec:related}

Here we cover other works that highlight adversarial examples and attacks leveraging them, in which their discoveries inspired our work.

\noindent{\bf Physical Adversarial Examples}

Athalye~\textit{et~al.}\cite{Athalye2017} suggested an algorithm for training adversarial examples robust to noise and arbitrary transformation. Brown~\textit{et~al.}\cite{Brown2017} applied this idea to create Adversarial Patches, which was adapted by Eykholt~\textit{et~al.}\cite{Eykholt2018} to fool object detectors. Our research attempts to take adversarial examples for ECGs to a similar direction as Eykholt's work, by implementing a physical method in which adversarial perturbations can be applied. 

\noindent{\bf Medical Adversarial Examples}

Finlayson~\textit{et~al.}\cite{Finlayson2019} shows that a trained classifier to diagnose medical images can be fooled by medical images perturbed by adversarial noise, or specifically trained patches applied on them, causing classifiers to make mistakes in diagnosing illnesses. Finlayson claimed that these examples threaten diagnosis systems, allowing adversaries to manipulate the outcome of diagnosis made by neural networks without directly tampering with the system itself, calling for infrastructural and algorithmic solutions~\cite{Finlayson2019}.

\noindent{\bf Attacks on ECGs}

We are not the first to formulate adversarial examples for ECGs. Chen~\textit{et~al.}\cite{Chen2019} shows  that classifiers trained to detect atrial fibrillation in ECG segments can be fooled by perturbing the original ECG. Han~\textit{et~al.}\cite{Han2019} explores how adversarial noise can be made undetectable, even to the eyes of a trained physician. Our research creates adversarial perturbations to attack ECGs in the context of beat-by-beat classification. We believe the difference in the steps taken to process the ECGs and the context under which they are diagnosed has a substantial influence on how the adversarial examples would have to be constructed and implemented to result in a meaningful attack. 
% \mori{本研究はend-to-end のハードウェア実験による real-world での評価も行っていることが大きな差分だと強調しましょう}
Furthermore, our work presents a real-world perspective of the threat of adversarial examples of ECGs by implementing them in an end-to-end hardware attack.

\noindent{\bf Injecting Signal in Physical Realm}

% \sugawara{
Related to our work on testing adversarial examples on a real ECG, there is a line of studies on attacking medical devices by injecting signals to their sensors in the physical realm.
% }
Kune~\textit{et~al.}\cite{Kune2013} explores the physical aspect of attacks on ECGs, and leverages electromagnetic interference (EMI) injection to perturb pace-maker readings, showing that hardware manipulation threatens ECG measurement systems.
%
% \sugawara{
Following this work, Tu~\textit{et~al.}~\cite{DBLP:conf/ccs/TuRHRFH19} formulate an attack against an infant incubator by injecting a fake signal to a temperature sensor with EMI; meanwhile, Park~\textit{et~al.}~\cite{DBLP:conf/woot/ParkSSKK16}
propose attacks on an infusion pump by shining infrared light to its drop sensor. See \cite{DBLP:journals/cacm/FuX18,DBLP:journals/corr/abs-1901-06935} for a complete survey.
% }


